High-Resolution Range-Doppler Imaging from One-Bit PMCW Radar via Generative Adversarial Networks

Digital modulation schemes such as PMCW have recently attracted increasing attention as possible replacements for FMCW modulation in future automotive radar systems. A significant obstacle to their widespread adoption is the expensive and power-consuming ADC required at gigahertz frequencies. To mitigate these challenges, employing low-resolution ADC, such as one-bit, has been suggested. Nonetheless, using one-bit sampling results in the loss of essential information. This study explores two RD imaging methods in PMCW radar systems utilizing NN. The first method merges standard RD signal processing with a GAN, whereas the second method uses an E2E strategy in which traditional signal processing is substituted with an NN-based RD module. The findings indicate that these methods can substantially improve the probability of detecting targets in the range-Doppler domain.

==> images/eval_range.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
\definecolor{mycolor4}{rgb}{0.49400,0.18400,0.55600}%
\definecolor{mycolor5}{rgb}{0.46600,0.67400,0.18800}%
\definecolor{mycolor6}{rgb}{0.30100,0.74500,0.93300}%
\definecolor{mycolor7}{rgb}{0.63500,0.07800,0.18400}%

\begin{axis}[
height=6cm,
width=\columnwidth,
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xmin=-1.91117691975, xmax=40.13471531475,
xtick style={color=black},
y grid style={darkgray176},
ytick style={color=black},
xlabel={Range bin $k$},
ylabel={Norm. power $\hat{q}\left[k, 256\right]$ (\SI{}{\decibel})},
xmax = 150,
xmin = 0,
ymax = 0,
ymin = -60,
ymajorgrids,
xmajorgrids,
legend style={legend cell align=left, draw=white!15!black}
]

\addplot [thick, mycolor1]
table {%
0 -45.4710706132528
1 -44.9945711404764
2 -56.3057288071645
3 -53.2132752705245
4 -48.9746415929062
5 -55.6923278859188
6 -45.3750372434712
7 -61.2490623252706
8 -51.2601166338196
9 0
10 -50.4794846806998
11 -46.9979344438379
12 -50.2881350767628
13 -51.3248239411746
14 -58.8753344199352
15 -46.9151038101582
16 -45.4212624341971
17 -45.7060927128633
18 -58.1258677218142
19 -52.3865270625872
20 -48.9985846770907
21 -45.6042086516221
22 -50.2709172922898
23 -50.218634356695
24 -53.9265123945152
25 -67.2101949995865
26 -66.1136904351114
27 -57.1946084739385
28 -47.8577024863104
29 -50.6284355056797
30 -52.7743384818644
31 -45.2145673897918
32 -46.8031079714173
33 -59.1639188089104
34 -55.202570862932
35 -53.2101899026154
36 -50.7760952811688
37 -45.618371744462
38 -50.6968437324368
39 -47.4883871806284
40 -57.2292039285237
41 -56.8579628667926
42 -52.012191597934
43 -56.5298263456977
44 -43.4200270980195
45 -48.9966608064533
46 -53.2451646863306
47 -51.416853110934
48 -42.0076222943443
49 -49.0063816364945
50 -45.0936307725993
51 -48.2994826153237
52 -53.2986071816306
53 -43.5580404295548
54 -60.0831114566451
55 -53.8803754186489
56 -50.4636420934145
57 -42.2926848351963
58 -52.9630127158852
59 -46.962721618907
60 -42.5637530282886
61 -47.3559681742427
62 -49.0239365304485
63 -46.5263971537063
64 -53.3334248964313
65 -42.2997571965783
66 -46.8763773958307
67 -43.2784623754676
68 -60.3035702259659
69 -52.8986502593002
70 -47.123557552323
71 -58.0517075980909
72 -51.5879342139456
73 -50.2982774399548
74 -47.5001380520781
75 -48.7548496157171
76 -49.6386732955839
77 -40.7030285812509
78 -45.5036931612285
79 -49.0254037896806
80 -52.017696054802
81 -45.4267215345879
82 -57.8828155987614
83 -50.7515234176766
84 -49.8159995130388
85 -46.9245660272994
86 -53.7178620142807
87 -50.1029526951854
88 -49.7776135946349
89 -56.971896238219
90 -59.4097419906184
91 -47.682517873747
92 -44.8527209471702
93 -49.7951787754234
94 -46.0506878256148
95 -45.725596329122
96 -52.5665852726114
97 -56.1546293190745
98 -56.0825701831743
99 -57.7349144572111
100 -65.2405002062622
101 -46.7747601572754
102 -48.8469917426677
103 -51.5975992791134
104 -48.4452621495555
105 -49.6388441011465
106 -50.1725941595339
107 -42.565944736751
108 -48.2659615572312
109 -60.800048175518
110 -50.5617833405264
111 -51.3509769127698
112 -50.406325152402
113 -55.0002822767911
114 -44.279717678759
115 -41.547398991834
116 -59.036572145548
117 -51.0501196887562
118 -45.7979142471365
119 -47.7342671907032
120 -50.0977521716978
121 -49.9157636104556
122 -59.947340575155
123 -49.3686031538723
124 -56.0124775621319
125 -45.9873392995799
126 -53.3095195240214
127 -47.957027875516
128 -52.0290250584016
129 -44.0112495138912
130 -48.4670955330439
131 -44.5129460386142
132 -41.6657341873745
133 -51.1955478885773
134 -47.5538829035705
135 -54.6926650597701
136 -48.14120616362
137 -53.3488884285621
138 -42.167939131916
139 -49.6131540601224
140 -43.7440055925743
141 -48.7641268115204
142 -42.2611212441177
143 -48.9705190947643
144 -51.5689317982959
145 -43.0710393372636
146 -46.1931397088322
147 -54.0158054452389
148 -51.3819478870851
149 -49.6021729575281
150 -47.8354032191266
151 -48.9552687985882
152 -49.5047920088095
153 -52.7967946296923
154 -60.1576534813244
155 -50.3407150437522
156 -53.7280774574496
157 -52.5041903314627
158 -54.3927936398984
159 -50.7187094332115
160 -53.2874843498721
161 -46.9096873260453
162 -52.6778776698284
163 -50.2934445086242
164 -54.9872146423328
165 -54.2009632411116
166 -63.2265989249901
167 -49.6692433789628
168 -49.6696757258223
169 -50.7955914546167
170 -45.8726625070242
171 -50.3981329011566
172 -53.1115200584189
173 -48.4813987061719
174 -50.5188406274143
175 -50.2952840809983
176 -54.6581309474874
177 -61.9010543926589
178 -54.1025684915439
179 -62.0907738238052
180 -52.4863828296853
181 -51.4579464368088
182 -47.0986138281627
183 -55.4790419809962
184 -48.5190157210496
185 -49.5967491435436
186 -46.781497555552
187 -49.4402939087792
188 -43.7972743550654
189 -54.312481466707
190 -50.3007627858956
191 -48.549248023004
192 -51.5478613861136
193 -55.7374651400215
194 -55.6067895792905
195 -60.6985759136888
196 -58.0667522325711
197 -44.8624731527568
198 -47.1810273447061
199 -55.8614523066144
200 -46.0898288845827
201 -61.0795712913403
202 -58.7452658900467
203 -45.8474395368928
204 -49.9024023158373
205 -57.5781259536525
206 -49.4816417987916
207 -63.8959868983537
208 -48.743342774268
209 -50.8177361446736
210 -44.5317200516942
211 -48.344808212578
212 -48.224525052592
213 -49.788676735846
214 -49.7574338441831
215 -49.5030719673491
216 -65.8897344818105
217 -53.1185331009786
218 -46.3382805965443
219 -49.1141411576664
220 -46.1246079606537
221 -46.8878094688811
222 -44.1346057502469
223 -50.3368837553536
224 -45.8973733788377
225 -55.7445202964739
226 -57.7339720602172
227 -46.898376614219
228 -48.7970164003116
229 -57.4376183289158
230 -53.4091178828424
231 -56.474185993366
232 -47.2517401269111
233 -65.2692464868566
234 -46.1146346062589
235 -56.6519394760188
236 -44.4017392446274
237 -59.5093507710245
238 -54.9101520228416
239 -46.7209165910114
240 -49.5362663033943
241 -61.459306100383
242 -50.660336597919
243 -46.5081282623599
244 -47.7168899727549
245 -44.2856825803919
246 -50.3296448246548
247 -47.830247743294
248 -55.7731131316788
249 -46.9745815218
250 -44.6392661518574
251 -49.0061196819049
252 -41.2872153333272
253 -61.7906282112349
254 -47.015026929663
255 -57.4828004564887
};
\addlegendentry{\glsxtrshort{WF}~1}

\addplot [thick, mycolor2]
table {%
0 -63.4341769202327
1 -48.4340160448286
2 -50.0065773247516
3 -47.8459290008507
4 -53.0600527188525
5 -48.8144660588873
6 -50.7483604208998
7 -49.833862761798
8 -54.3304817032139
9 -59.8634257688717
10 -45.8376331243368
11 -52.9951943941224
12 -50.8061245688065
13 -52.0561772464633
14 -49.1821151346707
15 -50.4671592594341
16 -47.9516526142993
17 -48.8950858342653
18 -43.8398262204509
19 -56.2169180575109
20 -49.2609986352908
21 -43.0841205993352
22 -44.3236631761335
23 -43.9301941741028
24 -49.2644694883467
25 -55.9145480281237
26 -57.2218448192968
27 -44.2994310137702
28 -50.0647843404649
29 -48.6541195643582
30 -48.9853101889911
31 -51.5444770009927
32 -53.6257942646199
33 -58.7781048742267
34 -51.5777577015811
35 -51.4061147215929
36 -49.894684471757
37 -45.6676772679388
38 -58.3375383860846
39 -54.0980044994704
40 -44.8153966563392
41 -61.0238417940859
42 -65.6249225362857
43 -42.1598074284199
44 -43.5877556925258
45 -57.0252480627021
46 -43.9308592055778
47 -51.7185117294865
48 -77.16289779236
49 -46.2015789988092
50 -53.1001409893657
51 -47.8379789711402
52 -51.1777395821651
53 -51.8851988202977
54 -47.6904103824139
55 -44.2939594906589
56 -51.8364638309769
57 -51.2490940088153
58 -44.7056884681697
59 -54.2991130869199
60 -44.2327127599085
61 -48.1619699767383
62 -65.9623872064185
63 -49.7699037320525
64 -46.4590798942667
65 -46.3755959388028
66 -49.0975898106508
67 -48.1279892347953
68 -47.0562152973202
69 -48.7134091308277
70 -51.4091194724731
71 -46.483088293408
72 -54.1913600150891
73 -50.849054134889
74 -49.8485743917395
75 -48.7509405801672
76 -53.5244103069556
77 -53.2482732409948
78 -42.9413742520472
79 -46.4600558884376
80 -48.1922634339082
81 -52.5765342980771
82 -48.1005034786211
83 -48.7586161265982
84 -52.2753138829877
85 -44.716267974075
86 -46.9190894521582
87 -16.8426091798324
88 -44.1338507454646
89 -50.9976264412112
90 -42.608419676688
91 0
92 -15.4225783915463
93 -49.7586855910128
94 -44.5809895094527
95 -54.1754414594915
96 -67.2588200740714
97 -49.0381382230419
98 -55.8180901326411
99 -58.3528175977345
100 -57.5135982886444
101 -52.5384649063603
102 -45.8131317064549
103 -55.226144609295
104 -47.8157253465985
105 -44.1911580037091
106 -49.6277330079992
107 -59.2543777451273
108 -51.6821570877605
109 -46.7988098058205
110 -49.3296061099434
111 -44.4338669886279
112 -43.5030711599772
113 -51.453017297202
114 -63.2984507782587
115 -41.3587810321831
116 -47.9762884757785
117 -53.3934136341092
118 -56.9988638843137
119 -47.9888369188843
120 -45.3035433073646
121 -40.4171280238644
122 -52.2936595928322
123 -50.0191364502794
124 -52.5792053353605
125 -54.2434665724695
126 -61.127969253947
127 -50.4196275080314
128 -49.5017357923774
129 -49.1071251496799
130 -53.9031724470898
131 -46.0174670083942
132 -50.785568240317
133 -50.2215236414037
134 -53.7832735802822
135 -42.340022564247
136 -45.702643771235
137 -43.8265699892199
138 -50.431472434152
139 -56.0359369517645
140 -50.2320958089062
141 -57.5956880363684
142 -48.3449973302365
143 -51.1228575635371
144 -48.8648000917407
145 -58.482894939808
146 -46.037632992901
147 -48.5074154187338
148 -44.8666341020234
149 -56.9384334856309
150 -47.5631424609604
151 -55.6480727150254
152 -43.6634295723326
153 -48.4114335660087
154 -64.7033005452127
155 -49.3666508304218
156 -48.8754247838384
157 -59.387256624728
158 -49.9052082625293
159 -43.9651815295378
160 -59.1796250323212
161 -43.8165894161101
162 -42.035921837744
163 -49.1605646670022
164 -46.6601258879668
165 -45.0560511651654
166 -53.7439810082826
167 -46.8012456142418
168 -56.8920549431055
169 -50.9002474322178
170 -48.6845887188032
171 -43.654130359992
172 -54.1722792044302
173 -50.4331148380297
174 -59.146301657551
175 -46.3556103179995
176 -46.3792262153072
177 -49.433646983542
178 -41.9623524506672
179 -49.1002158729561
180 -48.487725638201
181 -46.6692321925413
182 -50.1277510273504
183 -43.3489868990651
184 -45.8183255186276
185 -58.2897957535125
186 -47.275912604631
187 -61.8880808557763
188 -42.5609840720134
189 -51.6532868503242
190 -56.5339513767857
191 -46.9956986169848
192 -53.7594871264272
193 -44.0478014210889
194 -46.4320274504941
195 -50.3612504372231
196 -61.7644964495288
197 -41.8743754783465
198 -58.3903073963472
199 -50.0569226636371
200 -56.2307917638314
201 -59.5966114270185
202 -48.6060457338979
203 -46.5656517709061
204 -42.3360492400814
205 -44.2055615015588
206 -47.7391213874965
207 -49.2067327266658
208 -44.1060768106071
209 -45.4770795398831
210 -48.7952916104383
211 -43.485862570137
212 -52.4161420351045
213 -46.4144109040609
214 -43.6030551229267
215 -47.5584027449037
216 -50.3508239504203
217 -45.4197926475979
218 -58.4315915342403
219 -56.6131155981396
220 -50.3771347003843
221 -49.5776648682458
222 -44.9020436090601
223 -65.47782178354
224 -49.2528390387132
225 -47.204785268201
226 -52.9816609952992
227 -42.4685881947413
228 -50.9971481401033
229 -50.6452962774618
230 -47.2189122361505
231 -45.1244147088965
232 -52.2418332156627
233 -53.8969971143134
234 -56.0706141974861
235 -68.2827735107499
236 -42.3159081993936
237 -53.5810066323165
238 -52.3530332813818
239 -51.8664698746126
240 -48.0215678840717
241 -49.9101934071644
242 -52.8980742761347
243 -48.2560739598326
244 -53.9958065760817
245 -49.0404016839171
246 -41.9617976634358
247 -44.0225250015259
248 -55.5879562016812
249 -45.7901262029784
250 -50.2096339692678
251 -59.734912306159
252 -41.9998398392014
253 -53.4713020977341
254 -47.2783219932327
255 -48.5242037693433
};
\addlegendentry{\glsxtrshort{WF}~2}

\end{axis}

\end{tikzpicture}


==> images/eval_vel.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{mycolor1}{rgb}{0.00000,0.44700,0.74100}%
\definecolor{mycolor2}{rgb}{0.85000,0.32500,0.09800}%
\definecolor{mycolor3}{rgb}{0.92900,0.69400,0.12500}%
\definecolor{mycolor4}{rgb}{0.49400,0.18400,0.55600}%
\definecolor{mycolor5}{rgb}{0.46600,0.67400,0.18800}%
\definecolor{mycolor6}{rgb}{0.30100,0.74500,0.93300}%
\definecolor{mycolor7}{rgb}{0.63500,0.07800,0.18400}%

\begin{axis}[
height=4.5cm,
width=\columnwidth,
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xtick style={color=black},
y grid style={darkgray176},
ymin=-79.9847260269737, ymax=1.0,
ytick style={color=black},
xlabel={Doppler bin $m$},
ylabel={Norm. power $\hat{s}[9, m]$ (\SI{}{\decibel})},
xmax = 150,
xmin = 0,
ymax = 0,
ymin = -60,
ymajorgrids,
xmajorgrids,
legend style={legend cell align=left, draw=white!15!black}
]

\addplot [thick, mycolor5]
table {%
0 -41.6092041542341
1 -38.0062033200041
2 -39.2271120785478
3 -39.1858319406784
4 -42.2303209815117
5 -45.3609423589034
6 -40.0704283551228
7 -42.2194892315328
8 -49.349920702926
9 -49.7927193638558
10 -40.799522351786
11 -41.8387690415686
12 -49.3392480413825
13 -55.7297881440655
14 -67.3294876462676
15 -50.3612802090624
16 -44.3974880581453
17 -43.2879621408679
18 -43.4833790647365
19 -42.9506476574526
20 -44.8162847908708
21 -53.3208672229796
22 -40.125168210966
23 -41.7742302248296
24 -45.7137598478592
25 -44.6711011784106
26 -48.5234690608038
27 -56.7431145155973
28 -41.6348971375835
29 -42.544179479458
30 -47.7350045285798
31 -40.7333674804913
32 -44.0901256432942
33 -37.4761617473024
34 -36.6719524281821
35 -22.1135137802917
36 -2.83504931185073
37 0
38 -8.14774114511163
39 -28.1815866297952
40 -22.2715317044037
41 -10.3899462206918
42 -13.1488256948758
43 -33.0008749128812
44 -44.2604114081086
45 -53.9996540890199
46 -45.7260044548928
47 -47.2871035966344
48 -48.4192361637419
49 -47.7506397635708
50 -43.8371636923169
51 -49.4790413952164
52 -51.12692357434
53 -46.1841983867517
54 -42.635554081274
55 -45.1256001914609
56 -45.5548127317387
57 -50.5481173829992
58 -52.325142481692
59 -52.3745854612756
60 -50.1841508294929
61 -45.7043549369961
62 -46.4143031786272
63 -47.9109848819023
64 -44.5766413076465
65 -48.2949256457948
66 -50.8626364704521
67 -44.2810158159068
68 -51.4626294829755
69 -41.9856634356634
70 -37.9507904712298
71 -43.6951794798294
72 -40.8035492546788
73 -37.0223459496775
74 -37.2685313174051
75 -45.0110121469793
76 -41.068364197852
77 -43.203443800244
78 -43.0450278795222
79 -41.2687020237566
80 -46.9720812281246
81 -58.3756200016644
82 -51.1410825341963
83 -44.4882920745282
84 -41.1022290306369
85 -42.975012550937
86 -40.0595951977388
87 -38.6332979469149
88 -42.2965088940952
89 -50.8756790147394
90 -49.2371223567225
91 -41.4824751792953
92 -42.5110996432374
93 -45.1109180139245
94 -56.3449777304097
95 -45.1977329021913
96 -42.3021290915416
97 -42.0888932236802
98 -52.8785032168098
99 -41.0028932847783
100 -38.0439111014207
101 -39.3872125776201
102 -41.4910445733771
103 -42.8678577468632
104 -41.3849299368811
105 -39.4675773891147
106 -40.95318986495
107 -41.3042832474333
108 -40.0247639072575
109 -40.9372573968561
110 -42.4171096154611
111 -42.4985544863506
112 -38.4972312809016
113 -36.9225376366113
114 -41.0987617521568
115 -45.3201571968581
116 -51.1439077491368
117 -47.2685397290765
118 -47.7923255881708
119 -44.1597095727279
120 -50.5609572643069
121 -48.6690464538391
122 -48.1940281261169
123 -57.6495283448771
124 -50.2681632273487
125 -52.3669399409813
126 -47.0979464130996
127 -61.7043775893833
128 -51.415211090711
129 -59.1998499644162
130 -46.0728875933709
131 -58.2890830361992
132 -47.6160685172302
133 -44.4290591494326
134 -46.0210259020457
135 -53.6655497108395
136 -51.1844653134861
137 -41.7402129296056
138 -40.0545258867876
139 -44.4094333535463
140 -42.9823139911839
141 -46.6179049553952
142 -36.7896286377048
143 -37.0198855759381
144 -39.2162919126941
145 -44.5656931973092
146 -51.5967908281642
147 -43.703984061084
148 -55.989518259136
149 -52.1459034876388
150 -50.5948835830561
151 -42.3733327115124
152 -41.5952753652679
153 -48.335576584927
154 -63.8855272941926
155 -67.1093982441213
156 -71.7006610160438
157 -53.2137627012799
158 -43.3752174434355
159 -41.3191137935253
160 -42.3235178443062
161 -44.7930437125479
162 -45.4743364306322
163 -42.7134749733279
164 -46.4939323635768
165 -55.3830494102863
166 -49.3493792022795
167 -49.0425580196917
168 -42.3746126611926
169 -46.1925965722658
170 -49.5129964422695
171 -53.1180914570523
172 -43.3635852780812
173 -46.0535918691175
174 -46.5538135034888
175 -55.5305543452135
176 -51.7189479418721
177 -52.939971334157
178 -50.6724157101028
179 -47.4213117213363
180 -40.27326793824
181 -38.9278311768845
182 -41.3342956436365
183 -39.0694445987674
184 -39.4075545897317
185 -52.5479928758125
186 -49.5643690125105
187 -46.9457688711819
188 -43.7460218195913
189 -47.8393210141142
190 -47.371957564204
191 -46.3570673076623
192 -46.7766256603918
193 -45.2668874891885
194 -40.3205885548179
195 -41.1575521835228
196 -44.7853429866066
197 -45.2827108479334
198 -42.9672703055058
199 -44.0949809458804
200 -55.8068056251701
201 -48.6452396685513
202 -47.7082929988869
203 -47.3330259135325
204 -50.2401473786254
205 -42.9550058240985
206 -41.2493054465052
207 -45.8268546039066
208 -48.7205373606536
209 -47.9150970070204
210 -42.9762943903393
211 -40.5011487636787
212 -42.4504694762126
213 -54.1732427847916
214 -49.0801695611591
215 -45.713923503028
216 -42.8620488065451
217 -45.5531052018959
218 -42.9204481427195
219 -45.8065641284325
220 -52.0655098533228
221 -45.5570308358548
222 -43.9505992456737
223 -50.4135812903751
224 -46.5449590236286
225 -42.5258126602562
226 -43.1250383644191
227 -68.6233793661661
228 -48.5637900902316
229 -45.2996005018251
230 -49.4048959224402
231 -51.8344546884214
232 -50.7510267828786
233 -45.0522465119132
234 -48.4235951789659
235 -48.651234176856
236 -42.8735953555928
237 -42.257111326531
238 -46.7001368761748
239 -46.2785839259346
240 -44.8389047626968
241 -47.8244718128947
242 -43.0441543550751
243 -46.8418761712537
244 -45.7667771628358
245 -49.0787700939181
246 -42.2061515487444
247 -40.0728083016322
248 -47.8583929082149
249 -44.4429757882979
250 -45.8431052316227
251 -41.268948334521
252 -39.414199051538
253 -41.974007416843
254 -44.2185056400751
255 -47.6827582854015
};
\addlegendentry{\glsxtrshort{WF}~4}

\addplot [thick, mycolor7]
table {%
0 -65.0537061594229
1 -47.5804242653764
2 -41.5515692341494
3 -47.1081976070427
4 -45.2326905033303
5 -52.4951989913822
6 -53.8799087021381
7 -60.1292878996592
8 -43.206214504273
9 -40.0752193596798
10 -59.1493895643726
11 -44.1995537175265
12 -47.9161592748634
13 -58.8221991711496
14 -48.3286273604505
15 -44.5533321101461
16 -43.69255652298
17 -44.7854588527575
18 -47.6956383174969
19 -47.6270712062706
20 -48.5155990146789
21 -37.6678196824019
22 -37.4216755506774
23 -37.9787883864903
24 -35.7921098985588
25 -38.5693711355901
26 -60.6579055800498
27 -54.9572066189477
28 -37.1928962706004
29 -37.557851083662
30 -38.4224740272225
31 -41.4163144601251
32 -40.1319417198622
33 -38.5084824565592
34 -37.8472590644132
35 -23.6543682684686
36 -3.29285462760615
37 0
38 -7.47851668737584
39 -29.7619476594054
40 -21.5568127461635
41 -11.636722272874
42 -14.2912219707282
43 -37.106045845904
44 -36.8606168631214
45 -47.1875891412319
46 -51.6557220795298
47 -41.4964882960162
48 -46.7162347973775
49 -50.1183420587846
50 -47.4959067731965
51 -48.0844141965846
52 -44.936170613341
53 -46.1060764628928
54 -45.6865461337254
55 -42.6836139442053
56 -41.395684663177
57 -43.8735635911929
58 -47.3389934249777
59 -46.6710656168178
60 -64.3232133121958
61 -41.1660332158059
62 -39.7873337417695
63 -46.8806600109845
64 -43.0722527687455
65 -47.7856105635852
66 -53.4547766333973
67 -45.027798522194
68 -36.3072799785098
69 -36.3219301943491
70 -41.1055374381258
71 -43.6081544933773
72 -40.0224089071865
73 -40.8338165458723
74 -56.250759845546
75 -41.8127919707366
76 -46.8634804268961
77 -44.9878513309111
78 -45.8156576887815
79 -40.7116792913446
80 -39.8843833131477
81 -55.0622679176311
82 -41.1817979637447
83 -43.8532642912927
84 -45.8862460342307
85 -41.3560168197711
86 -46.4059540518419
87 -43.6096340394681
88 -40.4957636860273
89 -48.8193467096149
90 -38.3803684885965
91 -43.338965603538
92 -39.8465441762124
93 -43.5111093603317
94 -49.9227014200219
95 -39.8224461694207
96 -39.7347818225638
97 -41.1369060100766
98 -40.2359375724322
99 -41.7431330939496
100 -46.5528147167459
101 -47.2020003008295
102 -43.8961570094582
103 -47.4125618706217
104 -63.0714969570153
105 -48.1853303348801
106 -49.3414421791205
107 -48.8483043013118
108 -61.0263958502752
109 -48.7017546154119
110 -46.7175083181044
111 -41.7666284906892
112 -41.175031627678
113 -40.5615164855832
114 -35.3864917689628
115 -39.6547630305119
116 -41.2160614551305
117 -41.3853234517219
118 -45.1726044809198
119 -49.1875830717736
120 -58.853451199538
121 -67.7910498118331
122 -50.1091256370613
123 -50.32674451426
124 -50.9986977083909
125 -48.5423376736738
126 -48.4657760081142
127 -44.6628714470726
128 -45.7893320443809
129 -60.9203077202366
130 -50.8703892152062
131 -40.1707339015634
132 -42.834604458425
133 -50.7166940871832
134 -44.4587782421905
135 -38.6589672495568
136 -37.4084922894327
137 -40.6564713879444
138 -51.7907110058436
139 -50.778271799339
140 -48.0348402597663
141 -50.8035434520502
142 -67.2619266147535
143 -45.9951415595993
144 -49.0719552581333
145 -44.1384002877015
146 -41.2381559619093
147 -44.8570062219341
148 -37.5387700044044
149 -44.6374902988175
150 -43.3355946239459
151 -43.7073422090154
152 -46.4672517857839
153 -55.2814957660645
154 -50.540572625965
155 -45.2435175403963
156 -53.33730134144
157 -43.6112716692919
158 -56.5021570947655
159 -44.176612407486
160 -43.976717656621
161 -38.5182849004669
162 -41.9630559603238
163 -49.0471346024999
164 -42.4097139668019
165 -42.5156924172449
166 -45.8490406985501
167 -49.6400673222814
168 -48.1996978792608
169 -44.7551057427702
170 -43.7603985361973
171 -44.1782880733718
172 -45.7853679028016
173 -45.8545635899754
174 -50.05284183478
175 -46.6765511808683
176 -39.9845769558094
177 -41.7688447490789
178 -44.6354838412839
179 -58.6633499479669
180 -46.8426687063024
181 -51.4140542304977
182 -52.6670560637945
183 -46.0786908123054
184 -43.1924363609577
185 -43.4047471053492
186 -58.4427582815846
187 -44.7322834938771
188 -41.3724789289644
189 -38.6879943444207
190 -43.7746778904317
191 -46.700951602366
192 -47.1384109208303
193 -47.1286596564078
194 -41.8093338924226
195 -51.1849226698428
196 -39.4278689273029
197 -38.0110375137684
198 -43.5175808528589
199 -58.9259117347436
200 -52.0087494781881
201 -43.8920794267786
202 -51.0756082345844
203 -44.1602803189473
204 -40.424879154023
205 -40.9147481284617
206 -42.4700015459423
207 -42.6035428025686
208 -42.625593492555
209 -51.3345081113056
210 -41.848803232996
211 -41.0099133086152
212 -43.01156817961
213 -38.9814394853876
214 -41.3749193332942
215 -49.8138288791788
216 -44.9218464615502
217 -50.7001281262274
218 -41.8289089568686
219 -45.4228553430379
220 -49.2802772097764
221 -41.3314349721851
222 -43.911820399096
223 -40.7708718924137
224 -43.8570391162172
225 -40.8060703164581
226 -38.6647034953671
227 -47.8355806934668
228 -41.180261543679
229 -43.6934568602274
230 -46.0280015645008
231 -40.8968557293665
232 -39.7194425276151
233 -48.6765773035995
234 -45.4491413501863
235 -59.1257616491371
236 -39.6510489956157
237 -38.052318886227
238 -38.8080734588184
239 -41.2241111129982
240 -41.7875219965719
241 -50.2546779837187
242 -42.5185592798492
243 -34.1950305829673
244 -35.6946983316014
245 -46.9578575053217
246 -43.7141157244859
247 -38.9833693130738
248 -39.1812164530706
249 -40.5979696090588
250 -51.7474465891601
251 -46.559971505148
252 -41.4343121724806
253 -43.0250535025474
254 -56.425808755784
255 -58.1068034475233
};
\addlegendentry{\glsxtrshort{WF}~5}

\end{axis}

\end{tikzpicture}

